Quasi-Monte Carlo Graph Random Features

We present a novel mechanism to improve the accuracy of the recently-introduced class of graph random features (GRFs). Our method induces negative correlations between the lengths of the algorithm's random walks by imposing antithetic termination: a procedure to sample more diverse random walks which may be of independent interest. It has a trivial drop-in implementation. We derive strong theoretical guarantees on the properties of these quasi-Monte Carlo GRFs (q-GRFs), proving that they yield lower-variance estimators of the 2-regularised Laplacian kernel under mild conditions. Remarkably, our results hold for any graph topology. We demonstrate empirical accuracy improvements on a variety of tasks including a new practical application: time-efficient approximation of the graph diffusion process. To our knowledge, q-GRFs constitute the first rigorously studied quasi-Monte Carlo scheme for kernels defined on combinatorial objects, inviting new research on correlations between graph random walks.

==> applications.tex <==
\section{Applications}
\label{sec:app}

\subsection{Regularized Laplacian kernels and graph diffusion processes \textcolor{red}{(shall we move this later?)}}
Consider the $d$-regularised Laplacian kernels $\mathrm{K}: \mathcal{V} \times \mathcal{V} \rightarrow \mathbb{R}$ from \citep{graph_features}, given by the kernel matrix for some $d \in \mathbb{N}$ as follows:
\begin{equation}
\mathbf{K} = (\mathbf{I}_{N} + \sigma^{2}\mathbf{L})^{-d}.
\end{equation}
We will show now the close connection between regularised Laplacian kernels and graph diffusion processes. In the Euclidean $\mathbb{R}^{d}$-space, the \textit{diffusion process} is defined by the following \textit{heat equation}:
\begin{equation}
\frac{d\mathbf{u}}{dt} = \nabla^{2}\mathbf{u}    
\end{equation}
for the \textit{Laplacian} $\nabla^{2}=\frac{\partial^2 }{\partial x_{1}^2}+\frac{\partial^2 }{\partial x_{2}^2}+...\frac{\partial^2 }{\partial x_{n}^2}$ and with initial condition: $\mathbf{u}_{0} \in \mathbb{R}^{d}$. When the Euclidean space is replaced by the graph structure, $\nabla^{2}$ needs to be replaced by the negated graph Laplacian $-\mathbf{L}$ \textcolor{red}{\citep{...}}. We thus get the following differential equation:
\begin{equation}
\label{eq:diffusion}
\frac{d\mathbf{u}}{dt} = -\mathbf{L}\mathbf{u}    
\end{equation}
with the exact solution of the form: $\mathbf{u}_{t}=\exp(-t\mathbf{L})\mathbf{u}_{0}$. The matrix $\mathbf{K}^{\mathrm{diff}}_{t}=\exp(-t\mathbf{L})\mathbf{u}_{0}$ is often referred to as the \textit{graph diffusion kernel matrix} and it effectively defines the \textit{graph diffusion kernel}.

Upon discretization with the backward Euler step (which in general is much more stable than its forward analogue), we obtain for the discretization step $\delta t >0$:
\begin{equation}
\frac{\mathbf{u}_{\delta t} - \mathbf{u}_{0}}{\delta t} = -\mathbf{L}\mathbf{u}_{\delta t},    
\end{equation}
which leads to the following formula for: $\mathbf{u}_{\delta t}$:
\begin{equation}
\mathbf{u}_{\delta t} = (\mathbf{I}_{N}+\delta t \mathbf{L})^{-1}\mathbf{u}_{0}    
\end{equation}

==> graph_figure.tex <==
\pgfdeclarelayer{foreground layer}
    \pgfsetlayers{main,foreground layer}
    \begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
        \begin{pgfonlayer}{foreground layer}      
        \foreach [count=\i] \coord in {(7.56, 4.05),(7.7, 3.69)}{
        \node[main,thick,fill=white] (\i) at \coord {};}
        
        \node[main,thick,fill=yellow] (3) at (5.98,3.8) {i};

        \newcount\mycount;
        \foreach [count=\i] \coord in {(9.94, 2.97),(6.14, 2.61),(7.51, 3.33),(7.975, 2.97),(3.525, 3.33),(2.48, 2.97),(3.94, 2.97),(3.39, 2.97),(3.665, 2.61),(7.975, 2.61),(6.855, 2.25),(1.55, 2.97),(1.825, 2.61),(5.325, 2.97),(4.975, 1.89),(4.045, 2.25),(8.545, 2.61),(8.545, 2.25),(9.115, 1.89),(9.665, 2.25),(9.665, 1.89),(0.65, 2.97),(0.515, 2.61),(1.065, 2.25),(0.135, 2.25),(1.48, 1.89),(1.095, 1.53),(3.685, 2.25),(7.74, 1.89),(7.13, 1.53),(6.115, 1.89),(8.735, 1.53),(0.41, 1.89),(9.285, 1.17),(9.665, 1.53),(5.335, 1.89),(5.545, 1.53),(6.285, 1.17),(9.71, 0.81),(4.595, 1.17),(5.335, 0.81),(4.955, 0.45),(7.51, 0.81),(6.75, 0.45),(9.435, 0.45),(10.215, 1.53),(2.755, 2.61),(3.325, 2.25),(3.115, 2.61),(8.125, 0.09),(8.165, 1.17),(9.16, 0.81),(0.41, 1.53),(4.595, 0.45),(4.425, 1.53),(5.335, 0.45),(4.775, 0.09),(4.095, 0.09),(1.48, 1.53)}{
        \tikzmath{\mycount=\i+3;}
        \node[main,thick,fill=white] (\the\mycount) at \coord {};}
        \end{pgfonlayer}
        \draw[-] (2) -- (1);
\draw[thick,black!30,-] (2) -- (1);
\draw[thick,black!30,-] (3) -- (1);
\draw[thick,black!30,-] (4) -- (1);
\draw[thick,black!30,-] (5) -- (1);
\draw[thick,black!30,-] (5) -- (3);
\draw[thick,black!30,-] (5) -- (4);
\draw[thick,black!30,-] (6) -- (1);
\draw[thick,black!30,-] (6) -- (2);
\draw[thick,black!30,-] (7) -- (1);
\draw[thick,black!30,-] (7) -- (2);
\draw[thick,black!30,-] (7) -- (6);
\draw[thick,black!30,-] (9) -- (8);
\draw[thick,black!30,-] (10) -- (8);
\draw[thick,black!30,-] (11) -- (8);
\draw[thick,black!30,-] (12) -- (8);
\draw[thick,black!30,-] (12) -- (9);
\draw[thick,black!30,-] (12) -- (11);
\draw[thick,black!30,-] (13) -- (7);
\draw[thick,black!30,-] (13) -- (8);
\draw[thick,black!30,-] (14) -- (5);
\draw[thick,black!30,-] (14) -- (8);
\draw[thick,black!30,-] (15) -- (8);
\draw[thick,black!30,-] (16) -- (8);
\draw[thick,black!30,-] (16) -- (10);
\draw[thick,black!30,-] (16) -- (15);
\draw[thick,black!30,-] (17) -- (2);
\draw[thick,black!30,-] (17) -- (6);
\draw[thick,black!30,-] (18) -- (17);
\draw[thick,black!30,-] (19) -- (17);
\draw[thick,black!30,-] (20) -- (3);
\draw[thick,black!30,-] (21) -- (13);
\draw[thick,black!30,-] (21) -- (20);
\draw[thick,black!30,-] (22) -- (4);
\draw[thick,black!30,-] (22) -- (14);
\draw[thick,black!30,-] (22) -- (20);
\draw[thick,black!30,-] (22) -- (21);
\draw[thick,black!30,-] (24) -- (23);
\draw[thick,black!30,-] (26) -- (9);
\draw[thick,black!30,-] (26) -- (15);
\draw[thick,black!30,-] (26) -- (25);
\draw[thick,black!30,-] (27) -- (9);
\draw[thick,black!30,-] (27) -- (15);
\draw[thick,black!30,-] (27) -- (16);
\draw[thick,black!30,-] (27) -- (25);
\draw[thick,black!30,-] (27) -- (26);
\draw[thick,black!30,-] (28) -- (25);
\draw[thick,black!30,-] (29) -- (9);
\draw[thick,black!30,-] (29) -- (15);
\draw[thick,black!30,-] (29) -- (16);
\draw[thick,black!30,-] (29) -- (25);
\draw[thick,black!30,-] (29) -- (26);
\draw[thick,black!30,-] (29) -- (27);
\draw[thick,black!30,-] (30) -- (9);
\draw[thick,black!30,-] (30) -- (16);
\draw[thick,black!30,-] (30) -- (26);
\draw[thick,black!30,-] (30) -- (27);
\draw[thick,black!30,-] (30) -- (28);
\draw[thick,black!30,-] (30) -- (29);
\draw[thick,black!30,-] (31) -- (5);
\draw[thick,black!30,-] (31) -- (10);
\draw[thick,black!30,-] (31) -- (12);
\draw[thick,black!30,-] (31) -- (16);
\draw[thick,black!30,-] (32) -- (6);
\draw[thick,black!30,-] (32) -- (7);
\draw[thick,black!30,-] (32) -- (10);
\draw[thick,black!30,-] (32) -- (13);
\draw[thick,black!30,-] (32) -- (31);
\draw[thick,black!30,-] (33) -- (7);
\draw[thick,black!30,-] (33) -- (13);
\draw[thick,black!30,-] (33) -- (14);
\draw[thick,black!30,-] (33) -- (18);
\draw[thick,black!30,-] (33) -- (21);
\draw[thick,black!30,-] (34) -- (3);
\draw[thick,black!30,-] (34) -- (5);
\draw[thick,black!30,-] (34) -- (14);
\draw[thick,black!30,-] (34) -- (19);
\draw[thick,black!30,-] (34) -- (21);
\draw[thick,black!30,-] (35) -- (4);
\draw[thick,black!30,-] (35) -- (21);
\draw[thick,black!30,-] (35) -- (22);
\draw[thick,black!30,-] (35) -- (24);
\draw[thick,black!30,-] (35) -- (34);
\draw[thick,black!30,-] (36) -- (26);
\draw[thick,black!30,-] (36) -- (27);
\draw[thick,black!30,-] (37) -- (2);
\draw[thick,black!30,-] (37) -- (24);
\draw[thick,black!30,-] (37) -- (35);
\draw[thick,black!30,-] (38) -- (24);
\draw[thick,black!30,-] (40) -- (3);
\draw[thick,black!30,-] (40) -- (5);
\draw[thick,black!30,-] (40) -- (34);
\draw[thick,black!30,-] (40) -- (39);
\draw[thick,black!30,-] (41) -- (3);
\draw[thick,black!30,-] (41) -- (33);
\draw[thick,black!30,-] (41) -- (34);
\draw[thick,black!30,-] (41) -- (40);
\draw[thick,black!30,-] (42) -- (3);
\draw[thick,black!30,-] (42) -- (4);
\draw[thick,black!30,-] (42) -- (24);
\draw[thick,black!30,-] (42) -- (35);
\draw[thick,black!30,-] (42) -- (37);
\draw[thick,black!30,-] (43) -- (3);
\draw[thick,black!30,-] (43) -- (18);
\draw[thick,black!30,-] (43) -- (34);
\draw[thick,black!30,-] (43) -- (40);
\draw[thick,black!30,-] (44) -- (3);
\draw[thick,black!30,-] (44) -- (18);
\draw[thick,black!30,-] (44) -- (33);
\draw[thick,black!30,-] (44) -- (40);
\draw[thick,black!30,-] (44) -- (41);
\draw[thick,black!30,-] (45) -- (3);
\draw[thick,black!30,-] (45) -- (34);
\draw[thick,black!30,-] (45) -- (37);
\draw[thick,black!30,-] (45) -- (40);
\draw[thick,black!30,-] (45) -- (44);
\draw[thick,black!30,-] (46) -- (3);
\draw[thick,black!30,-] (46) -- (6);
\draw[thick,black!30,-] (46) -- (24);
\draw[thick,black!30,-] (46) -- (33);
\draw[thick,black!30,-] (46) -- (35);
\draw[thick,black!30,-] (46) -- (40);
\draw[thick,black!30,-] (46) -- (41);
\draw[thick,black!30,-] (47) -- (3);
\draw[thick,black!30,-] (47) -- (5);
\draw[thick,black!30,-] (47) -- (37);
\draw[thick,black!30,-] (47) -- (44);
\draw[thick,black!30,-] (48) -- (4);
\draw[thick,black!30,-] (48) -- (24);
\draw[thick,black!30,-] (48) -- (33);
\draw[thick,black!30,-] (48) -- (35);
\draw[thick,black!30,-] (48) -- (37);
\draw[thick,black!30,-] (48) -- (42);
\draw[thick,black!30,-] (49) -- (4);
\draw[thick,black!30,-] (49) -- (24);
\draw[thick,black!30,-] (50) -- (9);
\draw[thick,black!30,-] (51) -- (9);
\draw[thick,black!30,-] (51) -- (11);
\draw[thick,black!30,-] (51) -- (12);
\draw[thick,black!30,-] (52) -- (9);
\draw[thick,black!30,-] (53) -- (24);
\draw[thick,black!30,-] (53) -- (34);
\draw[thick,black!30,-] (53) -- (35);
\draw[thick,black!30,-] (53) -- (37);
\draw[thick,black!30,-] (53) -- (40);
\draw[thick,black!30,-] (53) -- (48);
\draw[thick,black!30,-] (54) -- (14);
\draw[thick,black!30,-] (54) -- (24);
\draw[thick,black!30,-] (54) -- (35);
\draw[thick,black!30,-] (55) -- (37);
\draw[thick,black!30,-] (56) -- (36);
\draw[thick,black!30,-] (57) -- (43);
\draw[thick,black!30,-] (58) -- (14);
\draw[thick,black!30,-] (58) -- (29);
\draw[thick,black!30,-] (59) -- (44);
\draw[thick,black!30,-] (60) -- (45);
\draw[thick,black!30,-] (60) -- (57);
\draw[thick,black!30,-] (61) -- (19);
\draw[thick,black!30,-] (61) -- (45);
\draw[thick,black!30,-] (62) -- (29);

\draw[red,very thick,-] (3) -- (40);
\draw[red,very thick,-] (40) -- (53);
\draw[red,very thick,-] (53) -- (48);
\draw[red,very thick,-] (48) -- (4);
\draw[red,very thick,-] (4) -- (49);
\draw[red,very thick,-] (49) -- (4);
\draw[red,very thick,-] (4) -- (48);
\draw[red,very thick,-] (48) -- (24);
\draw[red,very thick,-] (24) -- (37);
\draw[red,very thick,-] (37) -- (35);


\draw[red!40,very thick,-] (3) -- (1);
\draw[red!40,very thick,-] (1) -- (7);
\draw[red!40,very thick,-] (7) -- (2);
\draw[red!40,very thick,-] (2) -- (7);
\draw[red!40,very thick,-] (7) -- (32);
\draw[red!40,very thick,-] (32) -- (6);
\draw[red!40,very thick,-] (6) -- (46);

\draw[blue,very thick,-] (28) -- (25);
\draw[blue,very thick,-] (25) -- (29);
\draw[blue,very thick,-] (29) -- (15);
\draw[blue,very thick,-] (15) -- (29);
\draw[blue,very thick,-] (29) -- (15);
\draw[blue,very thick,-] (15) -- (8);
\draw[blue,very thick,-] (8) -- (14);
\draw[blue,very thick,-] (14) -- (33);
\draw[blue,very thick,-] (33) -- (14);
\draw[blue,very thick,-] (14) -- (5);
\draw[blue,very thick,-] (5) -- (3);

\draw[blue,very thick,-] (28) -- (25);
\draw[blue,very thick,-] (25) -- (26);
\draw[blue,very thick,-] (26) -- (30);
\draw[blue,very thick,-] (30) -- (27);
\draw[blue,very thick,-] (27) -- (16);
\draw[blue,very thick,-] (16) -- (15);
\draw[blue,very thick,-] (15) -- (26);
\draw[blue,very thick,-] (26) -- (29);
\draw[blue,very thick,-] (29) -- (16);

\draw[blue!50,very thick,-] (3) -- (18);
\draw[blue!50,very thick,-] (18) -- (43);
\draw[blue!50,very thick,-] (43) -- (57);

    \end{tikzpicture}

==> trv_offset.tex <==
\begin{tikzpicture}[baseline=(current  bounding  box.center), scale=0.5]
\def\eps{5}

\fill [fill=red!30] (0,0) rectangle (1,2);
\draw[very thick] (0,0)--(0,3);
\draw[very thick] (0,0)--(5,0);
\draw[black] (0,2)--(4,2)--(4,0);
\path (0,3) pic[rotate=180,scale=0.1] {arrowhead};
\path (5,0) pic[rotate=90,scale=0.1] {arrowhead};
\draw[very thick, ->] (0.9,0)--(0.9,1);
\draw[very thick, ->] (0.2,0)--(0.2,1);
\draw[very thick, ->] (2.3,0)--(2.3,1);
\node[scale=0.75] at (1,-0.5) {$p$};
\node[scale=0.75] at (4,-0.5) {$1$};
\node[scale=1] at (5.3,0) {$t$};

\def\eps{7}

\fill [fill=red!30] (\eps,0) rectangle (1+\eps,2);
\draw[very thick] (\eps,0)--(\eps,3);
\draw[very thick] (\eps,0)--(5+\eps,0);
\draw[black] (\eps,2)--(4+\eps,2)--(4+\eps,0);
\path (\eps,3) pic[rotate=180,scale=0.1] {arrowhead};
\path (5+\eps,0) pic[rotate=90,scale=0.1] {arrowhead};
\draw[very thick, ->] (0.4+\eps,0)--(0.4+\eps,1);
\draw[very thick, ->] (1.77+\eps,0)--(1.77+\eps,1);
\draw[very thick, ->] (3+\eps,0)--(3+\eps,1);
\node[scale=0.75] at (1+\eps,-0.5) {$p$};
\node[scale=0.75] at (4+\eps,-0.5) {$1$};
\node[scale=1] at (5.3+\eps,0) {$t$};

\draw [decorate,decoration = {brace,mirror}] (\eps + 1.77,-0.2) --  (3+\eps,-0.2);
\node[scale=0.75] at (1+\eps,-0.5) {$p$};
\node[scale=0.75] at (2.4+\eps,-0.8) {$\Delta=\frac{1}{3}$};
\end{tikzpicture}
